Secret Keepers: The Impact of LLMs on Linguistic Markers of Personal Traits

Prior research has established associations between individuals' language usage and their personal traits; our linguistic patterns reveal information about our personalities, emotional states, and beliefs. However, with the increasing adoption of Large Language Models (LLMs) as writing assistants in everyday writing, a critical question emerges: are authors' linguistic patterns still predictive of their personal traits when LLMs are involved in the writing process? We investigate the impact of LLMs on the linguistic markers of demographic and psychological traits, specifically examining three LLMs - GPT3.5, Llama 2, and Gemini - across six different traits: gender, age, political affiliation, personality, empathy, and morality. Our findings indicate that although the use of LLMs slightly reduces the predictive power of linguistic patterns over authors' personal traits, the significant changes are infrequent, and the use of LLMs does not fully diminish the predictive power of authors' linguistic patterns over their personal traits. We also note that some theoretically established lexical-based linguistic markers lose their reliability as predictors when LLMs are used in the writing process. Our findings have important implications for the study of linguistic markers of personal traits in the age of LLMs.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/F1_glms.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}[t]{lccccccc}
\toprule
  & Overall & Cohort & Conversations & Essays & Gender & YourMorals & Party\\
\midrule
(Intercept) & \num{-1.294}  *** & \num{-1.482}  *** & \num{-0.093} & \num{-0.656}  *** & \num{-1.359}  *** & \num{-0.617}  *** & \num{-1.519}  ***\\
 & {}[\num{-1.464}, \num{-1.127}] & {}[\num{-1.849}, \num{-1.132}] & {}[\num{-0.190}, \num{0.004}] & {}[\num{-0.757}, \num{-0.556}] & {}[\num{-1.652}, \num{-1.078}] & {}[\num{-0.729}, \num{-0.506}] & {}[\num{-1.932}, \num{-1.139}]\\
 & p = \num{<0.001} & p = \num{<0.001} & p = \num{0.060} & p = \num{<0.001} & p = \num{<0.001} & p = \num{<0.001} & p = \num{<0.001}\\
GPT & \num{0.254}  *** & \num{0.442} & \num{0.458}  *** & \num{0.141} & \num{0.223} & \num{0.176} & \num{0.770}  *\\
 & {}[\num{0.188}, \num{0.320}] & {}[\num{0.044}, \num{0.844}] & {}[\num{0.339}, \num{0.578}] & {}[\num{0.025}, \num{0.257}] & {}[\num{-0.097}, \num{0.548}] & {}[\num{0.043}, \num{0.309}] & {}[\num{0.300}, \num{1.259}]\\
 & p = \num{<0.001} & p = \num{0.030} & p = \num{<0.001} & p = \num{0.017} & p = \num{0.176} & p = \num{0.010} & p = \num{0.002}\\
LLama & \num{0.124}  ** & \num{0.030} & \num{0.028} & \num{0.213}  ** & \num{0.357} & \num{0.046} & \num{0.414}\\
 & {}[\num{0.056}, \num{0.192}] & {}[\num{-0.380}, \num{0.441}] & {}[\num{-0.090}, \num{0.147}] & {}[\num{0.094}, \num{0.333}] & {}[\num{0.040}, \num{0.679}] & {}[\num{-0.094}, \num{0.186}] & {}[\num{-0.073}, \num{0.918}]\\
 & p = \num{<0.001} & p = \num{0.886} & p = \num{0.640} & p = \num{<0.001} & p = \num{0.028} & p = \num{0.517} & p = \num{0.100}\\
SG & \num{0.062} & \num{0.354} & \num{-0.071} & \num{0.079} & \num{0.188} & \num{0.110} & \num{0.693}\\
 & {}[\num{0.009}, \num{0.116}] & {}[\num{0.028}, \num{0.683}] & {}[\num{-0.168}, \num{0.026}] & {}[\num{-0.014}, \num{0.171}] & {}[\num{-0.054}, \num{0.430}] & {}[\num{-0.002}, \num{0.223}] & {}[\num{0.189}, \num{1.212}]\\
 & p = \num{0.023} & p = \num{0.034} & p = \num{0.153} & p = \num{0.095} & p = \num{0.128} & p = \num{0.054} & p = \num{0.008}\\
Party & \num{0.205} &  &  &  &  &  & \\
 & {}[\num{0.005}, \num{0.407}] &  &  &  &  &  & \\
 & p = \num{0.046} &  &  &  &  &  & \\
Gender & \num{0.074} &  &  &  &  &  & \\
 & {}[\num{-0.126}, \num{0.277}] &  &  &  &  &  & \\
 & p = \num{0.471} &  &  &  &  &  & \\
Conversations & \num{1.169}  *** &  &  &  &  &  & \\
 & {}[\num{1.002}, \num{1.339}] &  &  &  &  &  & \\
 & p = \num{<0.001} &  &  &  &  &  \vphantom{2} & \\
Essays & \num{0.631}  *** &  &  &  &  &  & \\
 & {}[\num{0.465}, \num{0.800}] &  &  &  &  &  & \\
 & p = \num{<0.001} &  &  &  &  &  \vphantom{1} & \\
YourMorals & \num{0.651}  *** &  &  &  &  &  & \\
 & {}[\num{0.482}, \num{0.823}] &  &  &  &  &  & \\
 & p = \num{<0.001} &  &  &  &  &  & \\
\midrule
Num.Obs. & \num{22897} & \num{805} & \num{6557} & \num{7653} & \num{1372} & \num{5196} & \num{1314}\\
AIC & \num{30154.2} & \num{891.2} & \num{9022.9} & \num{10157.6} & \num{1574.0} & \num{6902.6} & \num{1566.2}\\
BIC & \num{30226.5} & \num{910.0} & \num{9050.0} & \num{10185.4} & \num{1594.9} & \num{6928.8} & \num{1597.3}\\
Log.Lik. & \num{-15068.095} & \num{-441.616} & \num{-4507.439} & \num{-5074.797} & \num{-782.997} & \num{-3447.310} & \num{-777.107}\\
RMSE & \num{0.48} & \num{0.43} & \num{0.50} & \num{0.48} & \num{0.44} & \num{0.49} & \num{0.45}\\
\bottomrule
\multicolumn{8}{l}{\rule{0pt}{1em}'*' =  0.00357, '**' = 0.0007, '***' = 0.00007.}\\
\end{tabular}}
\caption{Generalized linear models with the logit link predicting whether F1 scores remained constant/increased (1) or decreased (0) after LLM rewrite. $\alpha$ values were adjusted with Bonferroni corrections for multiple comparisons. The coefficients reflect the change in log odds of constant or increased F1 values.}
\end{table*}

==> tables/authority_corr.tex <==
\begin{table}[hbtp]
\centering
\resizebox{\textwidth}{!}{%
\centering
\begin{tabular}{rrr|rrrrrr|rrrrrr}
     & \multicolumn{2}{c}{ }& \multicolumn{6}{c}{Rewrite (R)} & \multicolumn{6}{c}{Syntax-Grammar (SG)} \\
      \cmidrule(lr){4-9}\cmidrule(l){10-15}
   & \multicolumn{2}{c}{Original}& \multicolumn{2}{c}{Gemini}& \multicolumn{2}{c}{GPT} &\multicolumn{2}{c}{Llama} & \multicolumn{2}{c}{Gemini}& 
   \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{Llama} \\
 & corr & p & corr & p & corr & p  & corr & p & corr & p & corr & p & corr & p\\ 
  \hline
i & \bf{0.07} & \bf{0.00} & \bf{0.07} & \bf{0.00} & \bf{0.09} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.08} & \bf{0.00} & \bf{0.07} & \bf{0.00} & \bf{0.11} & \bf{0.00} \\ 
  you & \bf{0.11} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.09} & \bf{0.00} & \bf{0.19} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.09} & \bf{0.00} & \bf{0.14} & \bf{0.00} \\ 
  pronoun & \bf{0.13} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.18} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.12} & \bf{0.00} \\ 
  affiliation & \bf{0.12} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.14} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.09} & \bf{0.00} & 0.10 & 0.00 \\ 
  Social & \bf{0.16} & \bf{0.00} & \bf{0.14} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.17} & \bf{0.00} & \bf{0.16} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.14} & \bf{0.00} \\ 
  prosocial & \bf{0.06} & \bf{0.00} & \bf{0.07} & \bf{0.00} & 0.05 & 0.00 & \bf{0.13} & \bf{0.00} & \bf{0.07} & \bf{0.00} & 0.06 & 0.00 & \bf{0.12} & \bf{0.00} \\ 
  relig & \bf{0.16} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.15} & \bf{0.00} & 0.06 & 0.06 & \bf{0.16} & \bf{0.00} & \bf{0.16} & \bf{0.00} & 0.09 & 0.00 \\ 
  Affect & \bf{0.15} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.25} & \bf{0.00} & \bf{0.16} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.15} & \bf{0.00} \\ 
  socrefs & \bf{0.16} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.14} & \bf{0.00} & \bf{0.19} & \bf{0.00} & \bf{0.16} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.12} & \bf{0.00} \\ 
  family & \bf{0.16} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.17} & \bf{0.00} & \bf{0.14} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.16} & \bf{0.00} & \bf{0.14} & \bf{0.00} \\ 
  friend & \bf{0.07} & \bf{0.00} & 0.06 & 0.00 & 0.05 & 0.01 & 0.08 & 0.01 & 0.06 & 0.00 & 0.04 & 0.01 & 0.07 & 0.02 \\ 
   \hline
\end{tabular}}
\caption{Pearson correlations between word frequencies and the moral foundation of Authority before and after LLM (Gemini, GPT, Llama) rewrite on the YourMorals dataset. Columns labeled R and SG indicate the ’rephrase’ and ’syntax-grammar’
conditions, respectively. Significant correlations are in bold (Bonferroni corrected p $\leq$ 0.000625).} 
\end{table}

==> tables/care_corr.tex <==
\begin{table}[ht!]
\centering
\resizebox{\textwidth}{!}{%
\centering
\begin{tabular}{rrr|rrrrrr|rrrrrr}
& \multicolumn{2}{c}{ }& \multicolumn{6}{c}{Rewrite (R)} & \multicolumn{6}{c}{Syntax-Grammar (SG)} \\
 \cmidrule(lr){4-9}\cmidrule(l){10-15}
 & \multicolumn{2}{c}{Original}& \multicolumn{2}{c}{Gemini}& \multicolumn{2}{c}{GPT} &\multicolumn{2}{c}{Llama} & \multicolumn{2}{c}{Gemini}& 
   \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{Llama} \\
 & corr & p & corr & p & corr & p  & corr & p & corr & p & corr & p & corr & p\\ 
  \hline
we & 0.03 & 0.05 & \bf{0.06} & \bf{0.00} & 0.05 & 0.00 & -0.01 & 0.87 & 0.05 & 0.00 & 0.03 & 0.07 & 0.04 & 0.24 \\ 
  pronoun & 0.03 & 0.06 & \bf{0.07} & \bf{0.00} & \bf{0.06} & \bf{0.00} & 0.08 & 0.01 & 0.04 & 0.03 & \bf{0.07} & \bf{0.00} & 0.06 & 0.05 \\ 
  affiliation & \bf{0.07} & \bf{0.00} & \bf{0.09} & \bf{0.00} & \bf{0.10} & \bf{0.00} & 0.06 & 0.07 & \bf{0.08} & \bf{0.00} & \bf{0.07} & \bf{0.00} & 0.07 & 0.02 \\ 
  Social & 0.05 & 0.00 & \bf{0.09} & \bf{0.00} & \bf{0.10} & \bf{0.00} & 0.07 & 0.01 & \bf{0.07} & \bf{0.00} & \bf{0.09} & \bf{0.00} & 0.08 & 0.01 \\ 
  socrefs & 0.05 & 0.01 & \bf{0.08} & \bf{0.00} & \bf{0.09} & \bf{0.00} & 0.09 & 0.00 & \bf{0.06} & \bf{0.00} & \bf{0.08} & \bf{0.00} & 0.07 & 0.04 \\ 
  family & 0.05 & 0.00 & 0.05 & 0.00 & \bf{0.07} & \bf{0.00} & 0.09 & 0.00 & \bf{0.06} & \bf{0.00} & \bf{0.06} & \bf{0.00} & 0.08 & 0.01 \\ 
  friend & 0.06 & 0.00 & \bf{0.06} & \bf{0.00} & \bf{0.07} & \bf{0.00} & 0.06 & 0.04 & 0.05 & 0.00 & 0.04 & 0.01 & 0.05 & 0.10 \\ 
   \hline
\end{tabular}}
\caption{Pearson correlations between word frequencies and the moral foundation of Care before and after LLM (Gemini, GPT, Llama) rewrite on the YourMorals dataset. Columns labeled R and SG indicate the ’rephrase’ and ’syntax-grammar’
conditions, respectively. Significant correlations are in bold (Bonferroni corrected p $\leq$ 0.000625).} 
\end{table}

==> tables/checkmark_empathy.tex <==
\begin{table*}[ht]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{llr|rrr|rrr}
&& \multicolumn{1}{c}{ }& \multicolumn{3}{c}{Rephrase (R)} & \multicolumn{3}{c}{Syntax-Grammar (SG)} \\
 \cmidrule(lr){4-6}\cmidrule(l){7-9}
 && \multicolumn{1}{c}{Original}& \multicolumn{1}{c}{Gemini}& \multicolumn{1}{c}{GPT3.5} &\multicolumn{1}{c}{Llama 2} & \multicolumn{1}{c}{Gemini}& 
   \multicolumn{1}{c}{GPT3.5} & \multicolumn{1}{c}{Llama 2} \\
  \hline
Personal Distress  &  Affect & \checkmark &  & & &   &   &  \\ 
          &  differ &  & & & \checkmark &  &   &  \\ 
   \hline
Empathetic Concern & cogproc & \checkmark &  &  & \checkmark&  &  &    \\ 
&  differ &  & &  & \checkmark& &   &    \\ 
   \hline
Perspective Taking & we & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
& pronoun & \checkmark & &  & \checkmark& \checkmark & &  \\ 
&  cogproc & &  &  \checkmark&\checkmark & &\\
   \hline
\end{tabular}}

\caption{Associations between LIWC categories and Interpersonality Reactivity Index (IRI) dimensions before and after ChatGPT rewrite on the Empathetic Conversations dataset. Columns labeled R and SG indicate the ’rephrase’ and ’syntax-grammar’ conditions, respectively. Significant correlations are indicated with a checkmark. Exact values and additional LIWC categories are reported in the appendices. The fourth dimension of the IRI, Fantasy, is not displayed as
no LIWC or empathy/distress lexicon categories were significantly correlated with this dimension.} 
\label{tab:checkmark-empathy}
\end{table*}


==> tables/correlation_big5.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{1.6cm}p{0.95cm}p{0.95cm}p{0.95cm}|p{0.95cm}p{0.95cm}p{0.95cm}|p{0.95cm}p{0.95cm}p{0.95cm}|p{0.95cm}p{0.95cm}p{0.95cm}|p{0.95cm}p{0.95cm}p{0.95cm}p{0.95cm}}
\toprule
  & \multicolumn{3}{c}{Openness}& \multicolumn{3}{c}{Conscientiousness}& \multicolumn{3}{c}{Extraversion} & \multicolumn{3}{c}{Agreeableness} & \multicolumn{4}{c}{Neuroticism} \\
  \hline
 Category&  & R& SG& & R& SG&  & R& SG&  & R& SG&  & R& \multicolumn{2}{l}{SG} \\
\hline
i & \textbf{-0.130}& \textbf{-0.110}& \textbf{-0.12}& 0.028& 0.019 & 0.030 & 0.060 & 0.054 & 0.068 & 0.053 & 0.036 & 0.038 & \textbf{0.150} & \multicolumn{2}{l}{\textbf{0.160}} & \textbf{0.140} \\
pronoun & -0.028 & 0.017 & 0.008 & 0.000 & -0.020 & -0.022 & 0.064 & 0.055 & 0.063 & 0.017 & -0.014 & -0.003 & \textbf{0.120} & \multicolumn{2}{l}{\textbf{0.110}} & \textbf{0.091} \\
affiliation & -0.057 & \underline{\textbf{-0.073}}& \underline{\textbf{-0.083}} & 0.048& 0.053 & \underline{\textbf{0.044}} & \textbf{0.110} & \textbf{0.110} & \textbf{0.110} & \textbf{0.078} & \textbf{0.088} & \textbf{0.083} & -0.012 & \multicolumn{2}{l}{-0.009} & -0.002 \\
achieve & -0.053 & \underline{\textbf{-0.084}} & \underline{\textbf{-0.08}} & 0.029& 0.023 & 0.031 & -0.002 & -0.009 & 0.011 & -0.025 & -0.019 & -0.022 & -0.001 & \multicolumn{2}{l}{-0.007} & -0.005 \\
Drives & -0.037 & \underline{\textbf{-0.073}} & \underline{\textbf{-0.073}} & 0.052& 0.041 & 0.044 & \textbf{0.091} & \textbf{0.073} & \textbf{0.089} & 0.043 & 0.051 & 0.042 & -0.017 & \multicolumn{2}{l}{-0.009} & -0.004 \\
Social & 0.057 & 0.045 & 0.051 & -0.025& -0.019 & -0.035 & \textbf{0.075} & \textbf{0.077} & \underline{0.064} & -0.005 & -0.004 & -0.011 & 0.021 & \multicolumn{2}{l}{0.011} & 0.026 \\
Affect & 0.027 & 0.002 & -0.005 & -0.061& -0.016 & -0.039 & 0.044 & \underline{\textbf{0.082}} & 0.066 & -0.049 & -0.006 & -0.025 & 0.057 & \multicolumn{2}{l}{\underline{\textbf{0.073}}} & \underline{\textbf{0.081}} \\
emotion & -0.047 & -0.036 & -0.039 & -0.003& 0.007 & -0.002 & 0.055 & \underline{\textbf{0.074}} & \underline{\textbf{0.075}} & 0.018 & 0.003 & 0.004 & \textbf{0.100} & \multicolumn{2}{l}{\textbf{0.120}} & \textbf{0.120} \\
emo.pos & -0.041 & -0.038 & -0.032 & 0.048& 0.055 & 0.043 & \textbf{0.096} & \textbf{0.120} & \textbf{0.110} & 0.063 & 0.062 & 0.054 & -0.050 & \multicolumn{2}{l}{-0.049} & -0.038 \\
emo.neg & -0.041 & -0.027 & -0.038 & -0.044& \underline{\textbf{-0.038}} & -0.044 & -0.027 & -0.012 & -0.004 & -0.042 & -0.050 & -0.043 & \textbf{0.190} & \multicolumn{2}{l}{\textbf{0.200}} & \textbf{0.210} \\
emo.anger & 0.000 & 0.031 & 0.017 & \textbf{-0.120}& \underline{-0.110} & \textbf{-0.120} & -0.026 & -0.032 & -0.029 & \textbf{-0.086} & \textbf{-0.110} & \textbf{-0.082} & \textbf{0.075} & \multicolumn{2}{l}{\underline{0.069}} & \underline{0.065} \\
emo.sad & 0.009 & 0.005 & -0.003 & 0.006& -0.009 & -0.007 & -0.006 & -0.007 & 0.013 & 0.021 & 0.039 & 0.045 & \textbf{0.100} & \multicolumn{2}{l}{\textbf{0.099}} & \textbf{0.100} \\
swear & \textbf{0.088} & \textbf{0.091} & \underline{0.068} & \textbf{-0.110}& \textbf{-0.073} & \textbf{-0.092} & -0.019 & -0.027 & -0.024 & \textbf{-0.120} & \underline{-}\underline{0.060} & \textbf{-0.084} & 0.003 & \multicolumn{2}{l}{0.013} & 0.006 \\
BigWords & \textbf{0.089} & \underline{0.002} & \underline{-0.009} & 0.030& 0.027 & 0.033 & -0.051 & -0.020 & -0.010 & -0.035 & 0.003 & -0.006 & -0.062 & \multicolumn{2}{l}{-0.039} & -0.016 \\
\midrule
Negative & 0.061 & -0.009 & 0.007 & -0.059& -0.061 & -0.057 & -0.061 & -0.055 & -0.039 & \textbf{-0.097} & \underline{-0.050} & \underline{-0.068} & 0.051 & \multicolumn{2}{l}{\underline{\textbf{0.094}}} & \underline{\textbf{0.076}} \\
Anger & 0.029 & -0.038 & -0.033 & -0.036& -0.038 & -0.029 & -0.009 & -0.010 & 0.000 & -0.053 & -0.015 & -0.029 & \textbf{0.075} & \multicolumn{2}{l}{\textbf{0.120}} & \textbf{0.100} \\
Anticipation & -0.044 & \underline{\textbf{-0.084}} & \underline{\textbf{-0.077}} & 0.042& 0.033 & 0.033 & 0.002 & 0.020 & 0.030 & \textbf{0.070} & \textbf{0.080} & \underline{0.062} & -0.022 & \multicolumn{2}{l}{-0.003} & 0.023 \\
Disgust & \textbf{0.092} & \underline{0.027} & \underline{0.029} & \textbf{-0.075}& \textbf{-0.079} & \textbf{-0.074} & -0.029 & -0.021 & -0.027 & \textbf{-0.081} & \underline{-0.047} & \underline{-0.065} & \textbf{0.069} & \multicolumn{2}{l}{\underline{0.066}} & \textbf{0.084} \\
Fear & 0.040 & -0.012 & -0.013 & -0.037& -0.031 & -0.026 & -0.033 & -0.005 & -0.007 & -0.023 & 0.011 & -0.002 & \textbf{0.110} & \multicolumn{2}{l}{\textbf{0.130}} & \textbf{0.130} \\
Joy & -0.033 & -0.056 & -0.057 & 0.034& 0.025 & 0.035 & \textbf{0.078} & \textbf{0.090} & \textbf{0.087} & 0.048 & 0.043 & 0.035 & -0.036 & \multicolumn{2}{l}{-0.012} & 0.004 \\
Sadness & 0.036 & -0.011 & 0.006 & \textbf{-0.071}& \underline{-0.066} & \underline{-0.049} & -0.060 & -0.042 & -0.021 & -0.034 & -0.036 & -0.036 & \textbf{0.130} & \multicolumn{2}{l}{\textbf{0.110}} & \textbf{0.097} \\
Trust & -0.051 & \underline{\textbf{-0.076}} & \underline{\textbf{-0.069}} & 0.002& 0.010 & 0.022 & 0.023 & 0.032 & 0.055 & 0.013 & 0.008 & 0.006 & -0.008 & \multicolumn{2}{l}{0.011} & 0.018 \\
\hline
\end{tabular}
}
\caption{Associations between word frequencies and Big Five Personality dimensions before and after ChatGPT rewrite on the Essays dataset. Columns labeled R and SG indicate the 'rephrase' and 'syntax-grammar' conditions, respectively. LIWC associations (Bonferroni corrected $p<$ 0.000714) are displayed in the top half, and NRC emotion lexicon ($p<$ 0.001) in the bottom half. Significant correlations are \textbf{boldfaced}, and correlations that became significant or lost significance after the rewrite are \underline{underlined}.}
\label{tab:correlation_big5}
\end{table*}

==> tables/correlation_empathy.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l l l l|l l l|l l l|l l l}
\toprule
  & \multicolumn{3}{c}{Concern} &\multicolumn{3}{c}{Fantasy}& \multicolumn{3}{c}{Perspective} & \multicolumn{3}{c}{Distress} \\
  \hline
 Category&  & R& SG& & R& SG&  & R& SG&  & R& SG\\
\hline
i.m & -0.017 & 0.015 & 0.021& 0.073 & 0.007 & 0.021 & \textbf{0.094} & \underline{0.000} & \underline{0.018} & \textbf{-0.220} & \underline{-0.043} & \underline{-0.057} \\
you.m & -0.009 & 0.018 & -0.010& -0.026 & -0.027 & 0.009 & 0.031 & -0.003 & 0.006 & \textbf{-0.100} & \underline{-0.030} & \underline{-0.012} \\
we.m & \textbf{-0.280} & \textbf{-0.140} & \textbf{-0.160}& \textbf{-0.270} & \underline{-0.068} & \underline{-0.082} & \textbf{-0.320} & \textbf{-0.150} & \textbf{-0.190} & \textbf{0.160} & \textbf{0.110} & \textbf{0.120} \\
shehe.m & \textbf{0.330} & \underline{0.090} & \underline{0.077}& -0.090 & -0.034 & -0.045 & \textbf{0.280} & \underline{0.080} & \underline{0.069} & -0.013 & 0.007 & -0.005 \\
they.m & -0.023 & 0.008 & 0.015& 0.047 & 0.047 & 0.05 & \textbf{-0.180} & \underline{-0.015} & \underline{-0.003} & -0.060 & -0.024 & -0.005 \\
pronoun.m & -0.230 & -0.087 & -0.077& -0.051 & -0.019 & -0.022 & \textbf{-0.350} & \textbf{-0.160} & \textbf{-0.130} & \textbf{0.120} & \underline{0.035} & \underline{0.010} \\
affiliation.m & -0.089 & -0.009 & -0.028& -0.007 & 0.006 & 0.014 & \textbf{-0.130} & \underline{0.010} & \underline{-0.031} & \textbf{0.110} & \underline{0.003} & \underline{0.011} \\
Social.m & \textbf{0.150} & \underline{0.057} & \underline{0.047}& \textbf{-0.130} & \underline{0.022} & \underline{0.028} & -0.007 & 0.042 & 0.034 & \textbf{0.250} & \underline{0.014} & \underline{0.003} \\
Affect.m & 0.010 & 0.063 & 0.047& 0.090 & 0.064 & 0.070 & \textbf{-0.200} & \underline{-0.010} & \underline{-0.013} & \textbf{0.180} & \underline{0.035} & \underline{0.025} \\
emo\_neg.m & \textbf{0.220} & \underline{0.086} & \underline{0.080}& \textbf{0.130} & \underline{0.047} & \underline{0.060} & -0.030 & 0.003 & 0.001 & 0.067 & 0.012 & -0.009 \\
cogproc.m & \textbf{-0.210} & \textbf{-0.100} & \textbf{-0.099}& -0.019 & -0.055 & -0.046 & \textbf{-0.290} & \textbf{-0.180} & \textbf{-0.140} & 0.032 & 0.055 & -0.011 \\
insight.m & -0.037 & -0.047 & -0.036& 0.080 & -0.013 & -0.016 & -0.081 & -0.065 & -0.059 & \textbf{-0.110} & \underline{0.016} & \underline{-0.027} \\
cause.m & 0.069 & 0.022 & -0.002& \textbf{0.230} & \underline{-0.005} & \underline{-0.010} & -0.014 & -0.032 & -0.033 & \textbf{-0.280} & \underline{-0.020} & \underline{-0.027} \\
tentat.m & \textbf{-0.200} & \textbf{-0.120} & \textbf{-0.120}& 0.006 & -0.091 & -0.08 & \textbf{-0.200} & \textbf{-0.110} & \textbf{-0.110} & 0.048 & 0.041 & 0.032 \\
differ.m & \textbf{-0.110} & \textbf{-0.092} & \textbf{-0.100}& -0.057 & -0.062 & -0.085 & -0.073 & \underline{\textbf{-0.100}} & \underline{\textbf{-0.110}} & \textbf{-0.110} & \underline{0.053} & \underline{0.021} \\
\bottomrule
\end{tabular}
}
\caption{Associations (Bonferroni corrected $p<$ 0.000781) between LIWC word frequencies and Interpersonal Reactivity Index (IRI) dimensions before and after ChatGPT rewrite on the Empathetic Conversations dataset. Columns labeled R and SG indicate the 'rephrase' and 'syntax-grammar' conditions, respectively. Significant correlations are \textbf{boldfaced}, and correlations that became significant or lost significance after the rewrite are \underline{underlined}.}
\label{tab:correlation_empathy}
\end{table*}

==> tables/correlation_moralvalues.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l l l l|l l l|l l l|l l l|l l l}
\toprule
  & \multicolumn{3}{c}{Care} & \multicolumn{3}{c}{Fairness} & \multicolumn{3}{c}{Loyalty} & \multicolumn{3}{c}{Purity} & \multicolumn{3}{c}{Authority} \\
  \hline
 Category&  & R& SG&   & R& SG&   & R& SG&   & R& SG&   & R& SG\\
\hline
i & 0.050 & 0.048 & \underline{\textbf{0.057}} & -0.006 & 0.013 & 0.01 & 0.027 & \underline{\textbf{0.063}} & 0.054 & \textbf{0.058} & \textbf{0.064} & \textbf{0.064} & \textbf{0.073} & \textbf{0.085} & \textbf{0.076} \\
you & 0.035 & 0.055 & \underline{\textbf{0.065}} & -0.014 & -0.005 & 0.013 & \textbf{0.082} & \textbf{0.086} & \textbf{0.097} & \textbf{0.130} & \textbf{0.110} & \textbf{0.120} & \textbf{0.110} & \textbf{0.086} & \textbf{0.089} \\
we & 0.033 & 0.050 & 0.030 & -0.049 & -0.024 & -0.032 & -0.004 & 0.023 & 0.014 & \textbf{0.071} & \textbf{0.085} & \textbf{0.065} & 0.036 & 0.046 & 0.039 \\
pronoun & 0.031 & \underline{\textbf{0.063}} & \underline{\textbf{0.073}} & -0.053 & -0.013 & -0.017 & 0.041 & \underline{\textbf{0.060}} & \underline{\textbf{0.077}} & \textbf{0.130} & \textbf{0.130} & \textbf{0.140} & \textbf{0.130} & \textbf{0.110} & \textbf{0.120} \\
affiliation & \textbf{0.074} & \textbf{0.100} & \textbf{0.073} & -0.04 & -0.009 & -0.020 & \textbf{0.065} & \textbf{0.080} & \underline{0.056} & \textbf{0.150} & \textbf{0.150} & \textbf{0.120} & \textbf{0.120} & \textbf{0.110} & \textbf{0.090} \\
Social & 0.051 & \underline{\textbf{0.099}} & \underline{\textbf{0.092}} & -0.045 & 0.011 & 0.021 & \textbf{0.083} & \textbf{0.100} & \textbf{0.110} & \textbf{0.190} & \textbf{0.180} & \textbf{0.180} & \textbf{0.160} & \textbf{0.120} & \textbf{0.120} \\
prosocial & 0.022 & 0.032 & 0.042 & -0.009 & 0.003 & 0.032 & 0.053 & \underline{\textbf{0.058}} & \underline{\textbf{0.070}} & \textbf{0.062} & \underline{0.054} & \textbf{0.062} & \textbf{0.064} & \underline{0.051} & \underline{0.056} \\
relig & -0.004 & 0.012 & 0.007 & \textbf{-0.063} & \underline{-0.052} & \textbf{-0.057} & \textbf{0.120} & \textbf{0.130} & \textbf{0.120} & \textbf{0.210} & \textbf{0.210} & \textbf{0.220} & \textbf{0.160} & \textbf{0.150} & \textbf{0.160} \\
Affect & 0.010 & 0.055 & 0.017 & -0.04 & 0.012 & -0.012 & \textbf{0.100} & \textbf{0.130} & \textbf{0.110} & \textbf{0.120} & \textbf{0.130} & \textbf{0.110} & \textbf{0.160} & \textbf{0.130} & \textbf{0.130} \\
socrefs & 0.046 & 0.094 & \underline{\textbf{0.079}} & -0.046 & -0.012 & -0.007 & \textbf{0.095} & \textbf{0.110} & \textbf{0.100} & \textbf{0.190} & \textbf{0.200} & \textbf{0.190} & \textbf{0.160} & \textbf{0.140} & \textbf{0.130} \\
family & 0.047 & 0.066 & 0.055 & -0.031 & -0.022 & -0.023 & \textbf{0.120} & \textbf{0.120} & \textbf{0.110} & \textbf{0.150} & \textbf{0.170} & \textbf{0.150} & \textbf{0.160} & \textbf{0.170} & \textbf{0.160} \\
friend & 0.055 & 0.065 & 0.044 & -0.004 & 0.011 & 0.004 & \textbf{0.075} & \underline{0.056} & \textbf{0.057} & \textbf{0.075} & \textbf{0.063} & \textbf{0.059} & 0.069 & 0.047 & 0.042 \\
\midrule
Virtue & \textbf{0.085} & \textbf{0.095} & \textbf{0.085} & 0.016 & 0.037 & 0.028 & -0.022 & 0.008 & -0.003 & \textbf{0.210} & \textbf{0.220} & \textbf{0.220} & \textbf{0.041} & \underline{0.003} & \underline{0.018} \\
Vice & 0.010 & 0.005 & -0.010 & 0.017 & 0.013 & 0.020 & 0.003 & 0.010 & 0.008 & \textbf{-0.061} & \underline{0.018} & \underline{-0.024} & \textbf{0.046} & \textbf{0.038} & \textbf{0.041} \\
\hline
\end{tabular}
}
\caption{Associations between word frequencies and Moral Foundations dimensions before and after ChatGPT rewrite on the YourMorals dataset. Columns labeled R and SG indicate the 'rephrase' and 'syntax-grammar' conditions, respectively. LIWC associations (Bonferroni corrected $p<$ 0.000625) are displayed in the top half, and MFD2 ($p<$ 0.025) in the bottom half. Significant correlations are \textbf{boldfaced}, and correlations that became significant or lost significance after the rewrite are \underline{underlined}.}
\label{tab:correlation_moralvalues}
\end{table*}

==> tables/fairness_corr.tex <==
\begin{table}[ht!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{rrr|rrrrrr|rrrrrr}
& \multicolumn{2}{c}{ }& \multicolumn{6}{c}{Rewrite (R)} & \multicolumn{6}{c}{Syntax-Grammar(SG)} \\
 \cmidrule(lr){4-9}\cmidrule(l){10-15}
& \multicolumn{2}{c}{Original}& \multicolumn{2}{c}{Gemini}& \multicolumn{2}{c}{GPT} &\multicolumn{2}{c}{Llama} & \multicolumn{2}{c}{Gemini}& 
   \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{Llama} \\
 & corr & p & corr & p & corr & p  & corr & p & corr & p & corr & p & corr & p\\ 
  \hline
pronoun & -0.05 & 0.00 & -0.03 & 0.13 & -0.01 & 0.45 & -0.02 & 0.49 & \bf{-0.06} & \bf{0.00} & -0.02 & 0.30 & -0.02 & 0.62 \\ 
  relig & \bf{-0.06} & \bf{0.00} & -0.03 & 0.04 & -0.05 & 0.00 & -0.01 & 0.75 & -0.05 & 0.00 & -0.06 & 0.00 & -0.02 & 0.52 \\ 
   \hline
\end{tabular}}
\caption{Pearson correlations between word frequencies and the moral foundation of Fairness before and after LLM (Gemini, GPT, Llama) rewrite on the YourMorals dataset. Columns labeled R and SG indicate the ’rephrase’ and ’syntax-grammar’
conditions, respectively. Significant correlations are in bold (Bonferroni corrected p $\leq$ 0.000625).} 
\end{table}


==> tables/loyalty_corr.tex <==
\begin{table}[ht!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{rrr|rrrrrr|rrrrrr}
     & \multicolumn{2}{c}{ }& \multicolumn{6}{c}{Rewrite (R)} & \multicolumn{6}{c}{Syntax-Grammar (SG)} \\
      \cmidrule(lr){4-9}\cmidrule(l){10-15}
   & \multicolumn{2}{c}{Original}& \multicolumn{2}{c}{Gemini}& \multicolumn{2}{c}{GPT} &\multicolumn{2}{c}{Llama} & \multicolumn{2}{c}{Gemini}& 
   \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{Llama} \\
 & corr & p & corr & p & corr & p  & corr & p & corr & p & corr & p & corr & p\\ 
  \hline
i & 0.03 & 0.11 & 0.03 & 0.04 & \bf{0.06} & \bf{0.00} & 0.10 & 0.00 & 0.04 & 0.03 & 0.05 & 0.00 & 0.11 & 0.00 \\ 
  you & \bf{0.08} & \bf{0.00} & \bf{0.10} & \bf{0.00} & \bf{0.09} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.09} & \bf{0.00} & \bf{0.10} & \bf{0.00} & \bf{0.12} & \bf{0.00} \\ 
  pronoun & 0.04 & 0.01 & 0.05 & 0.00 & \bf{0.06} & \bf{0.00} & \bf{0.14} & \bf{0.00} & 0.05 & 0.00 & \bf{0.08} & \bf{0.00} & 0.09 & 0.00 \\ 
  affiliation & \bf{0.06} & \bf{0.00} & \bf{0.10} & \bf{0.00} & \bf{0.08} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.07} & \bf{0.00} & 0.06 & 0.00 & 0.07 & 0.03 \\ 
  Social & \bf{0.08} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.10} & \bf{0.00} & \bf{0.17} & \bf{0.00} & \bf{0.10} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.12} & \bf{0.00} \\ 
  prosocial & 0.05 & 0.00 & \bf{0.07} & \bf{0.00} & \bf{0.06} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.06} & \bf{0.00} & \bf{0.07} & \bf{0.00} & \bf{0.11} & \bf{0.00} \\ 
  relig & \bf{0.12} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.13} & \bf{0.00} & 0.09 & 0.00 & \bf{0.12} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.11} & \bf{0.00} \\ 
  Affect & \bf{0.10} & \bf{0.00} & \bf{0.10} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.21} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.11} & \bf{0.00} \\ 
  socrefs & \bf{0.10} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.16} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.10} & \bf{0.00} & 0.09 & 0.00 \\ 
  family & \bf{0.11} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.12} & \bf{0.00} & 0.09 & 0.00 & \bf{0.11} & \bf{0.00} & \bf{0.11} & \bf{0.00} & 0.10 & 0.00 \\ 
  friend & \bf{0.07} & \bf{0.00} & \bf{0.06} & \bf{0.00} & 0.06 & 0.00 & 0.07 & 0.03 & \bf{0.06} & \bf{0.00} & 0.06 & 0.00 & 0.06 & 0.05 \\ 
   \hline
\end{tabular}}
\caption{Pearson correlations between word frequencies and the moral foundation of Loyalty before and after LLM (Gemini, GPT3.5, Llama) rewrite on the YourMorals dataset. Columns labeled R and SG indicate the ’rephrase’ and ’syntax-grammar’ conditions, respectively. Significant correlations are in bold (Bonferroni corrected p $\leq$ 0.000625).} 
\end{table}

==> tables/purity_corr.tex <==
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
\centering
\begin{tabular}{rrr|rrrrrr|rrrrrr}
& \multicolumn{2}{c}{ }& \multicolumn{6}{c}{Rewrite (R)} & \multicolumn{6}{c}{Syntax-Grammar (SG)} \\
\cmidrule(lr){4-9}\cmidrule(l){10-15}
 & \multicolumn{2}{c}{Original}& \multicolumn{2}{c}{Gemini}& \multicolumn{2}{c}{GPT} &\multicolumn{2}{c}{Llama} & \multicolumn{2}{c}{Gemini}& 
   \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{Llama} \\
 & corr & p & corr & p & corr & p  & corr & p & corr & p & corr & p & corr & p\\ 
  \hline
i & \bf{0.06} & \bf{0.00} & 0.04 & 0.01 & \bf{0.06} & \bf{0.00} & \bf{0.11} & \bf{0.00} & 0.05 & 0.00 & \bf{0.06} & \bf{0.00} & 0.11 & 0.00 \\ 
  you & \bf{0.13} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.17} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.15} & \bf{0.00} \\ 
  we & \bf{0.07} & \bf{0.00} & \bf{0.09} & \bf{0.00} & \bf{0.09} & \bf{0.00} & 0.07 & 0.03 & \bf{0.08} & \bf{0.00} & \bf{0.07} & \bf{0.00} & 0.02 & 0.53 \\ 
  pronoun & \bf{0.13} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.17} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.14} & \bf{0.00} & \bf{0.11} & \bf{0.00} \\ 
  affiliation & \bf{0.15} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.14} & \bf{0.00} & \bf{0.14} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.10} & \bf{0.00} \\ 
  Social & \bf{0.19} & \bf{0.00} & \bf{0.20} & \bf{0.00} & \bf{0.18} & \bf{0.00} & \bf{0.18} & \bf{0.00} & \bf{0.20} & \bf{0.00} & \bf{0.18} & \bf{0.00} & \bf{0.16} & \bf{0.00} \\ 
  prosocial & \bf{0.06} & \bf{0.00} & \bf{0.07} & \bf{0.00} & 0.05 & 0.00 & \bf{0.12} & \bf{0.00} & \bf{0.08} & \bf{0.00} & \bf{0.06} & \bf{0.00} & \bf{0.13} & \bf{0.00} \\ 
  relig & \bf{0.21} & \bf{0.00} & \bf{0.21} & \bf{0.00} & \bf{0.21} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.21} & \bf{0.00} & \bf{0.22} & \bf{0.00} & \bf{0.16} & \bf{0.00} \\ 
  Affect & \bf{0.12} & \bf{0.00} & \bf{0.12} & \bf{0.00} & \bf{0.13} & \bf{0.00} & \bf{0.20} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.11} & \bf{0.00} & \bf{0.12} & \bf{0.00} \\ 
  socrefs & \bf{0.19} & \bf{0.00} & \bf{0.20} & \bf{0.00} & \bf{0.20} & \bf{0.00} & \bf{0.19} & \bf{0.00} & \bf{0.20} & \bf{0.00} & \bf{0.19} & \bf{0.00} & \bf{0.13} & \bf{0.00} \\ 
  family & \bf{0.15} & \bf{0.00} & \bf{0.15} & \bf{0.00} & \bf{0.17} & \bf{0.00} & 0.10 & 0.00 & \bf{0.15} & \bf{0.00} & \bf{0.15} & \bf{0.00} & 0.10 & 0.00 \\ 
  friend & \bf{0.07} & \bf{0.00} & \bf{0.07} & \bf{0.00} & \bf{0.06} & \bf{0.00} & 0.08 & 0.01 & \bf{0.07} & \bf{0.00} & \bf{0.06} & \bf{0.00} & 0.10 & 0.00 \\ 
   \hline
\end{tabular}}
\caption{Pearson correlations between word frequencies and the moral foundation of Purity before and after LLM (Gemini, GPT3.5, Llama) rewrite on the YourMorals dataset. Columns labeled R and SG indicate the ’rephrase’ and ’syntax-grammar’
conditions, respectively. Significant correlations are in bold (Bonferroni corrected p $\leq$ 0.000625).} 
\end{table}

